High-Intensity Discharge Lamp and Duffing Oscillator - Similarities and Differences

The processes inside the arc tube of high-intensity discharge lamps are investigated by finite element simulations. The behavior of the gas mixture inside the arc tube is governed by differential equations describing mass, energy and charge conservation as well as the Helmholtz equation for the acoustic pressure and the Navier-Stokes equation for the flow driven by the buoyancy and the acoustic streaming force. The model is highly nonlinear and requires a recursion procedure to account for the impact of acoustic streaming on the temperature and other fields. The investigations reveal the presence of a hysteresis and the corresponding jump phenomenon, quite similar to a Duffing oscillator. The similarities and, in particular, the differences of the nonlinear behavior of the high-intensity discharge lamp to that of a Duffing oscillator are discussed. For large amplitudes the high-intensity discharge lamp exhibits a stiffening effect in contrast to the Duffing oscillator.

==> HIDLiteratur.tex <==
%% This BibTeX bibliography file was created using BibDesk.
%% http://bibdesk.sourceforge.net/


%% Created for Bernd Baumann at 2015-04-09 14:38:31 +0200 


%% Saved with string encoding Unicode (UTF-8) 



@article{schwiegercharacterization,
	Author = {Schwieger, Joerg and Wolff, Marcus and Baumann, Bernd and Manders, Freddy and Suijker, Jos},
	Date-Added = {2015-04-09 12:38:12 +0000},
	Date-Modified = {2015-04-09 12:38:12 +0000},
	Publisher = {IEEE},
	Title = {Characterization of Discharge Arc Flicker in High-Intensity Discharge Lamps}}

@article{hunt2006buckling,
	Author = {Hunt, Giles},
	Date-Added = {2015-01-22 13:37:49 +0000},
	Date-Modified = {2015-01-22 13:37:49 +0000},
	Journal = {Nonlinear Dynamics},
	Number = {1-2},
	Pages = {29--46},
	Publisher = {Springer},
	Title = {Buckling in space and time},
	Volume = {43},
	Year = {2006}}

@article{Benilov1998,
	Author = {Mikhail S. Benilov},
	Date-Added = {2015-01-06 09:47:13 +0000},
	Date-Modified = {2015-01-06 09:47:13 +0000},
	Journal = {Physical Review E},
	Number = {5},
	Pages = {6480-6494},
	Title = {Nonlinear surface heating of a plane sample and modes of current transfer to hot arc cathodes},
	Volume = {58},
	Year = {1998}}

@article{BenilovCunha2003,
	Author = {Mikhail S. Benilov and M{\'a}rio D. Cunha},
	Date-Added = {2015-01-06 09:42:32 +0000},
	Date-Modified = {2015-01-06 09:51:00 +0000},
	Journal = {Physical Review E},
	Number = {5},
	Pages = {056407},
	Title = {Bifurcation points in the theory of axially symmetric arc cathodes},
	Volume = {68},
	Year = {2003}}

@article{ising1925beitrag,
	Author = {Ising, Ernst},
	Date-Added = {2014-12-05 10:04:25 +0000},
	Date-Modified = {2014-12-05 10:04:25 +0000},
	Journal = {Zeitschrift f{\"u}r Physik A Hadrons and Nuclei},
	Number = {1},
	Pages = {253--258},
	Publisher = {Springer},
	Title = {Beitrag zur theorie des ferromagnetismus},
	Volume = {31},
	Year = {1925}}

@article{pelissetto2002critical,
	Author = {Pelissetto, Andrea and Vicari, Ettore},
	Date-Added = {2014-12-04 21:09:38 +0000},
	Date-Modified = {2014-12-04 21:09:38 +0000},
	Journal = {Physics Reports},
	Number = {6},
	Pages = {549--727},
	Publisher = {Elsevier},
	Title = {Critical phenomena and renormalization-group theory},
	Volume = {368},
	Year = {2002}}

@book{waymouth1971electric,
	Author = {Waymouth, John F},
	Date-Added = {2014-08-16 18:11:06 +0000},
	Date-Modified = {2014-08-16 18:11:06 +0000},
	Publisher = {MIT press Cambridge, MA},
	Title = {Electric discharge lamps},
	Volume = {168},
	Year = {1971}}

@conference{schwiegerinfluence,
	Address = {Rotterdam, Netherlands},
	Author = {Schwieger, J{\"o}rg and Baumann, Bernd and Wolff, Marcus and Manders, Freddy and Suijker, Jos},
	Booktitle = {Proc. COMSOL Users Conf.},
	Date-Added = {2014-07-31 12:50:26 +0000},
	Date-Modified = {2014-08-01 13:53:13 +0000},
	Title = {Influence of Thermal Conductivity and Plasma Pressure on Temperature Distribution and Acoustical Eigenfrequencies of High-Intensity Discharge Lamps},
	Year = {2013}}

@techreport{NEMA2010,
	Address = {Rosslyn, VA},
	Date-Added = {2014-07-31 12:18:11 +0000},
	Date-Modified = {2014-07-31 12:42:45 +0000},
	Institution = {National Bureau of Standards},
	Title = {The strength and potentials of metal halide lighting systems},
	Year = {2010}}

@article{Schuster.1940,
	Author = {K Schuster and W Matz},
	Date-Added = {2014-07-31 11:54:55 +0000},
	Date-Modified = {2014-07-31 18:25:33 +0000},
	Journal = {Akustische Zeitschrift},
	Pages = {349--352},
	Title = {{\"U}ber station{\"a}re {S}tr{\"o}mungen im {K}undtschen {R}ohr},
	Volume = {5},
	Year = {1940}}

@article{Rayleigh.1883,
	Author = {Lord Rayleigh},
	Date-Added = {2014-07-31 11:53:32 +0000},
	Date-Modified = {2014-07-31 18:37:19 +0000},
	Doi = {10.1098/rstl.1884.0002},
	Issn = {0261--0523},
	Journal = {Philosophical Transactions of the Royal Society of London},
	Number = {0},
	Pages = {1--21},
	Title = {On the circulation of air observed in {K}undt's tubes, and on some allied acoustical problems},
	Volume = {175},
	Year = {1883},
	Bdsk-Url-1 = {http://dx.doi.org/10.1098/rstl.1884.0002}}

@article{stockwald2014high,
	Author = {Stockwald, Klaus and Kaestle, Herbert and Ernst, Herbert},
	Date-Added = {2014-07-29 12:06:48 +0000},
	Date-Modified = {2014-07-29 12:06:48 +0000},
	Publisher = {IEEE},
	Title = {High Efficient Metal Halide HID Systems with Acoustically Stabilized Convection},
	Year = {2014}}

@inproceedings{stockwald2008significant,
	Author = {Stockwald, Klaus and Kaestle, Herbert and Weiss, Herbert},
	Booktitle = {Plasma Science, 2008. ICOPS 2008. IEEE 35th International Conference on},
	Date-Added = {2014-07-29 12:05:36 +0000},
	Date-Modified = {2014-07-29 12:05:36 +0000},
	Organization = {IEEE},
	Pages = {1--1},
	Title = {Significant efficacy enhancement of low wattage metal halide hid lamp systems by acoustically induced convection configuration},
	Year = {2008}}

@article{olsen2011experimental,
	Author = {Olsen, Jo and Dreeben, Thomas D},
	Date-Added = {2014-07-29 12:04:09 +0000},
	Date-Modified = {2014-07-29 12:04:09 +0000},
	Journal = {Industry Applications, IEEE Transactions on},
	Number = {1},
	Pages = {368--375},
	Publisher = {IEEE},
	Title = {Experimental and simulated straightening of metal halide arcs using power modulation},
	Volume = {47},
	Year = {2011}}

@techreport{PhilipsMaterialDatabase,
	Date-Added = {2014-07-24 14:25:05 +0000},
	Date-Modified = {2014-07-24 14:26:20 +0000},
	Institution = {Philips},
	Title = {Philips material database}}

@article{hust1984update,
	Author = {Hust, Jerome G and Lankford, Alan B},
	Date-Added = {2014-07-23 20:12:46 +0000},
	Date-Modified = {2014-07-31 12:37:30 +0000},
	Journal = {U. S. Dept. of Commerce},
	Pages = {61},
	Title = {Update of thermal conductivity and electrical resistivity of electrolytic iron, tungsten and stainless steel},
	Year = {1984}}

@book{cross2009pattern,
	Author = {Cross, Michael and Greenside, Henry},
	Date-Added = {2014-07-23 14:54:31 +0000},
	Date-Modified = {2014-07-23 14:54:31 +0000},
	Publisher = {Cambridge University Press},
	Title = {Pattern formation and dynamics in nonequilibrium systems},
	Year = {2009}}

@article{kreuzer1977physics,
	Author = {Kreuzer, Lloyd B},
	Date-Added = {2014-07-18 20:30:06 +0000},
	Date-Modified = {2014-07-18 20:30:06 +0000},
	Journal = {Optoacoustic Spectroscopy and Detection},
	Pages = {1--25},
	Publisher = {London, UK: Academic},
	Title = {The physics of signal generation and detection},
	Year = {1977}}

@article{boluriaan2003acoustic,
	Author = {Boluriaan, Said and Morris, Philip J},
	Date-Added = {2014-07-18 15:13:09 +0000},
	Date-Modified = {2014-07-31 18:34:19 +0000},
	Journal = {International Journal of aeroacoustics},
	Number = {3},
	Pages = {255--292},
	Publisher = {Multi-Science},
	Title = {Acoustic streaming: from {R}ayleigh to today},
	Volume = {2},
	Year = {2003}}

@book{temkin1981elements,
	Author = {Temkin, Samuel},
	Date-Added = {2014-07-18 14:55:55 +0000},
	Date-Modified = {2014-07-18 14:55:55 +0000},
	Publisher = {Wiley New York},
	Title = {Elements of acoustics},
	Year = {1981}}

@inproceedings{trestman2002minimizing,
	Author = {Trestman, Grigoriy A and Sylvania, Osram},
	Booktitle = {IECON 02 [Industrial Electronics Society, IEEE 2002 28th Annual Conference of the]},
	Date-Added = {2014-07-18 11:32:59 +0000},
	Date-Modified = {2014-07-18 11:32:59 +0000},
	Organization = {IEEE},
	Pages = {1214--1218},
	Title = {Minimizing cost of HID lamp electronic ballast},
	Volume = {2},
	Year = {2002}}

@book{waide2006light,
	Author = {Waide, Paul and Tanishima, Satoshi and Harrington, Phil},
	Date-Added = {2014-07-18 11:31:36 +0000},
	Date-Modified = {2014-07-18 11:31:36 +0000},
	Publisher = {OECD},
	Title = {Light's Labour's Lost: Policies for Energy-efficient Lighting},
	Year = {2006}}

@article{hamilton2003acoustic,
	Author = {Hamilton, Mark F and Ilinskii, Yurii A and Zabolotskaya, Evgenia A},
	Date-Added = {2014-07-18 11:26:53 +0000},
	Date-Modified = {2014-07-18 11:26:53 +0000},
	Journal = {The Journal of the Acoustical Society of America},
	Number = {1},
	Pages = {153--160},
	Publisher = {Acoustical Society of America},
	Title = {Acoustic streaming generated by standing waves in two-dimensional channels of arbitrary width},
	Volume = {113},
	Year = {2003}}

@article{dreeben2008modelling,
	Author = {Dreeben, Thomas D},
	Date-Added = {2014-07-18 11:03:22 +0000},
	Date-Modified = {2014-07-18 11:03:22 +0000},
	Journal = {Journal of Physics D: Applied Physics},
	Number = {14},
	Pages = {144023},
	Publisher = {IOP Publishing},
	Title = {Modelling of fluid-mechanical arc instability in pure-mercury HID lamps},
	Volume = {41},
	Year = {2008}}

@article{baumann2008modeling,
	Author = {Baumann, Bernd and Kost, Bernd and Wolff, Marcus and Groninga, Hinrich},
	Date-Added = {2014-07-18 10:54:24 +0000},
	Date-Modified = {2014-07-18 10:54:24 +0000},
	Journal = {Recent Advances in Modelling and Simulation},
	Pages = {17--38},
	Title = {Modeling and numerical investigation of photoacoustic resonators},
	Year = {2008}}

@inproceedings{baumann2007numerical,
	Author = {Baumann, Bernd and Kost, Bernd and Wolff, Marcus and Groninga, Hinrich and Bl{\"o}{\ss}, Tanja and Knickrehm, Stefan},
	Booktitle = {Proceedings of the European COMSOL Conference 2007},
	Date-Added = {2014-07-18 10:54:21 +0000},
	Date-Modified = {2014-07-18 10:54:21 +0000},
	Pages = {1--6},
	Title = {Numerical shape optimization of photoacoustic sample cells: first results},
	Year = {2007}}

@article{baumannfemlab,
	Author = {Baumann, B and Kost, B and Groninga, H and Wolff, M},
	Date-Added = {2014-07-18 10:54:19 +0000},
	Date-Modified = {2014-07-18 10:54:19 +0000},
	Title = {FEMLAB Konferenz}}

@article{baumanncomsol,
	Author = {Baumann, B and Kost, B and Wolff, M and Groninga, H and Bl{\"o}{\ss}, T and Knickrehm, S},
	Date-Added = {2014-07-18 10:54:17 +0000},
	Date-Modified = {2014-07-18 10:54:17 +0000},
	Title = {COMSOL Conference 2007}}

@article{kost2011numerical,
	Author = {Kost, B and Baumann, B and Germer, M and Wolff, M and Rosenkranz, M},
	Date-Added = {2014-07-18 10:54:14 +0000},
	Date-Modified = {2014-07-18 10:54:14 +0000},
	Journal = {Applied physics B},
	Number = {1},
	Pages = {87--93},
	Publisher = {Springer},
	Title = {Numerical shape optimization of photoacoustic resonators},
	Volume = {102},
	Year = {2011}}

@article{baumann2007solving,
	Author = {Baumann, Bernd and Wolff, Marcus and Kost, Bernd and Groninga, Hinrich},
	Date-Added = {2014-07-18 10:54:12 +0000},
	Date-Modified = {2014-07-18 10:54:12 +0000},
	Journal = {The International Journal of Multiphysics},
	Number = {3},
	Pages = {303--316},
	Publisher = {Multi-Science},
	Title = {Solving a coupled field problem by eigenmode expansion and finite element method},
	Volume = {1},
	Year = {2007}}

@article{baumann2007finite,
	Author = {Baumann, Bernd and Wolff, Marcus and Kost, Bernd and Groninga, Hinrich},
	Date-Added = {2014-07-18 10:54:10 +0000},
	Date-Modified = {2014-07-18 10:54:10 +0000},
	Journal = {Applied Optics},
	Number = {7},
	Pages = {1120--1125},
	Publisher = {Optical Society of America},
	Title = {Finite element calculation of photoacoustic signals},
	Volume = {46},
	Year = {2007}}

@article{baumann2006eigenmode,
	Author = {Baumann, Bernd and Kost, Bernd and Groninga, Hinrich and Wolff, Marcus},
	Date-Added = {2014-07-18 10:54:06 +0000},
	Date-Modified = {2014-07-18 10:54:06 +0000},
	Journal = {Review of Scientific Instruments},
	Number = {4},
	Pages = {044901},
	Publisher = {AIP Publishing},
	Title = {Eigenmode analysis of photoacoustic sensors via finite element method},
	Volume = {77},
	Year = {2006}}

@article{wolff2005resonance,
	Author = {Wolff, Marcus and Groninga, Hinrich G and Baumann, Bernd and Kost, Bernd and Harde, Hermann},
	Date-Added = {2014-07-18 10:54:02 +0000},
	Date-Modified = {2014-07-18 10:54:02 +0000},
	Journal = {Acta Acustica},
	Number = {Suppl 1},
	Pages = {99},
	Title = {Resonance Investigations using PAS and FEM},
	Volume = {91},
	Year = {2005}}

@article{afshar2008theory,
	Author = {Afshar, Farhang},
	Date-Added = {2014-07-18 10:30:34 +0000},
	Date-Modified = {2014-07-18 10:30:34 +0000},
	Journal = {Leukos},
	Number = {1},
	Pages = {27--38},
	Publisher = {Taylor \&amp; Francis},
	Title = {The theory of acoustic resonance and acoustic instability in HID lamps},
	Volume = {5},
	Year = {2008}}

@article{zissis2010diagnostics,
	Author = {Zissis, Georges and Haverlag, Marco},
	Date-Added = {2014-07-16 09:48:58 +0000},
	Date-Modified = {2014-07-16 09:48:58 +0000},
	Journal = {Journal of Physics D: Applied Physics},
	Number = {23},
	Pages = {230301},
	Publisher = {IOP Publishing},
	Title = {Diagnostics for electrical discharge light sources: pushing the limits},
	Volume = {43},
	Year = {2010}}

@article{baumann2009finite,
	Author = {Baumann, Bernd and Wolff, Marcus and Hirsch, John and Antonis, Piet and Bhosle, Sounil and Barrientos, Ricardo Valdivia},
	Date-Added = {2014-06-30 15:00:58 +0000},
	Date-Modified = {2014-06-30 15:00:58 +0000},
	Journal = {Journal of Physics D: Applied Physics},
	Number = {22},
	Pages = {225209},
	Publisher = {IOP Publishing},
	Title = {Finite element estimation of acoustical response functions in HID lamps},
	Volume = {42},
	Year = {2009}}

@article{hirsch2010acoustic,
	Author = {Hirsch, John and Baumann, Bernd and Wolff, Marcus and Bhosle, Sounil and Barrientos, Ricardo Valdivia},
	Date-Added = {2014-06-30 15:00:46 +0000},
	Date-Modified = {2014-06-30 15:00:46 +0000},
	Journal = {Journal of Physics D: Applied Physics},
	Number = {23},
	Pages = {234002},
	Publisher = {IOP Publishing},
	Title = {Acoustic resonances in HID lamps: model and measurement},
	Volume = {43},
	Year = {2010}}

